Linear Additive Markov Processes

We introduce LAMP: the Linear Additive Markov Process. Transitions in LAMP may be influenced by states visited in the distant history of the process, but unlike higher-order Markov processes, LAMP retains an efficient parametrization. LAMP also allows the specific dependence on history to be learned efficiently from data. We characterize some theoretical properties of LAMP, including its steady-state and mixing time. We then give an algorithm based on alternating minimization to learn LAMP models from data. Finally, we perform a series of real-world experiments to show that LAMP is more powerful than first-order Markov processes, and even holds its own against deep sequential models (LSTMs) with a negligible increase in parameter complexity.

==> app.tex <==
\appendix

\iffalse

\section{Growth Rates and Mixing Times}
We provide full proofs from Section \ref{concrete-growth-rates} The form of Bernstein's inequality used is:

\begin{thm}[Bernstein's inequality]
\label{thm:bernstein}
Let $X_1, \ldots, X_n$ be independent, $0$-mean random variables
and let $|X_i| \leq M$ for all $i$. Then for all $r > 0$, 
$$\Pr\left[ \sum_{i=1}^n X_i > r \right] < 
\exp\left(\frac{-\frac{1}{2}r^2}
  {\sum E[X_j^2] + \frac{1}{3}Mr} \right).$$
\end{thm}

We define
\[
 C(\epsilon) =  \frac{\epsilon^2 E[w]} {(1 + \epsilon)(2 \var[w] +
   \frac{2}{3} k \epsilon E[w])}.
\]

and for ease of notation, let $a(t, \epsilon) = t/(1 + \epsilon)E[w]$.

\begin{proof}[Theorem 12]
  Note that $$\Pr[e_t < a(t, \epsilon) ] = \Pr[W_1 + \cdots +
  W_{a(t, \epsilon)} > t]. $$ In our setting, we let $W'_i = W_i -
  E[w]$.  
Applying Theorem~\ref{thm:bernstein},
\begin{eqnarray*}
\lefteqn{
\Pr \left[\sum_{i=1}^{a(t, \epsilon)} W_i > t\right] 
= \Pr \left[ \sum_{i=1}^{a(t, \epsilon)} W'_i \geq a(t, \epsilon)
  \cdot \epsilon \cdot  E[w] \right]} \\
& \leq & 
\exp\left( - \displaystyle{\frac{\frac{1}{2}(a(t, \epsilon) \cdot
      \epsilon \cdot  E[w])^2}{a(t, \epsilon) \var[w] + \frac{1}{3}k
      \cdot a(t, \epsilon) \cdot \epsilon E[w]}} \right) \\
& = & \exp\left(- \displaystyle{\frac{t \epsilon^2 E[w]}{(1 + \epsilon)(2 \var[w] + \frac{2}{3} k \epsilon E[w])}} \right) \\
& = & \exp \left( - C(\epsilon) \cdot t \right).
\end{eqnarray*}
%
Fixing $T$ large and applying a union bound,
$$\sum_{t \geq T} \Pr \left[ \sum_{i=1}^{a(t, \epsilon)} W_i > t
\right]  \leq \sum_{t > T}  e^{-C(\epsilon) \cdot t} 
 = \frac{ e^{-C(\epsilon) \cdot T}} {1 - e^{-C(\epsilon)}}.
\qed
$$
\end{proof}

For the infinite $k$ case, we adapt a version of Markov inequality.
%
\begin{thm}[Fourth moment inequality]
\label{thm:markov}
Let $X$ be a nonnegative
random variable, with $E[|X|^4] < \infty$.  Then for all
$r > 0$,
$$ \Pr[ |X - E[X]| > r ] \leq \frac{E[(X - E[X])^4]}{r^4}.$$
\end{thm}

\begin{proof}[Theorem 14]
Letting $W'_i = W_i - E[w]$.  
Now, as the $W'_i$ are independent and have 0 mean, 
$$ E \left[ \left( \sum_{i=1}^{a(t, \epsilon)} W'_i \right)^4 \right]
=
\sum_{i} E[W'_i]^4 + 
\binom{a(t, \epsilon)}{2} \sum_{i, j} E[W'_i]^2 E[W'_j]^2.$$
We then apply Theorem~\ref{thm:markov} to get
\begin{eqnarray*}
\lefteqn{
\Pr\left[ \sum_{i=1}^{a(t, \epsilon)} W_i > t \right]
= \Pr \left[ \sum_{i=1}^{a(t, \epsilon)} W'_i > \frac{\epsilon
    t}{1 + \epsilon} \right] } \\
& \leq & 
\left( a(t, \epsilon) E[W'^4] + a(t, \epsilon)^2 E[W'^2]^2 \right) 
  \cdot \frac{(1 + \epsilon)^4}{\epsilon^4 t^4} \\
& = & \frac{(1 + \epsilon)^3}{\epsilon^4 t^3 E[w]} \cdot E[W'^4] + \frac{(1 + \epsilon)^2}{(E[w])^2 \epsilon^4 t^2} \cdot (E[W'^2])^2 \\
& = & \frac{D(\epsilon)}{t^2},
\end{eqnarray*}
where $D(\epsilon) < \infty$ is appropriately defined.  To get the
growth rate to hold for all $t \geq T$, we apply a union bound as
before
$$\sum_{t \geq T} \Pr\left[\sum_{i=1}^{a(t, \epsilon)} W'_i > \frac{\epsilon t}{1 + \epsilon} \right]
\leq \sum_{t \geq T} \frac{D(\epsilon)}{t^2} \leq
O\left(\frac{1}{T}\right).
\qed
$$
\end{proof}

\fi

\iftrue
% SORRY HAD TO HARDCODE BCOS OF LATEX BUG?
\section{Proof of Theorem 15}
\label{app:glamp}

Recall that $P = \sum_{i\in[k]} w_i P^{f(i)}$.
The proof has three parts.

(1) \textit{The equilibrium $\pi$ for $\GLAMP(w, \CP, f)$ is also the
  equilibrium for $P$:} Let $v_{ijtt^*}$ be the probability of
transitioning to $j$ at time $t^*$ from $i$ at time $t$. And
$v_{ijt^*} = \sum_{t < t^*} v_{ijtt^*}$ be the probability of
transitioning to $j$ at time $t^*$ from state $i$ at some time $t <
t^*$.  Then $v_{ijtt^*} = \pi_i w_{t^* - t} P^{f(t^* - t)}(i,j)$ where
$P^{f(t^* - t)}(i,j)$ is the $(i, j)$th entry of the matrix $P^{f(t^* -
  t)}$. So,
$$
v_{ijt^*} = 
\sum_{l = 1}^k \pi_i w_{t^* - l} P^{f(t^* - l)}(i,j)
% &= \pi_i \sum_{l = 1}^k w_{t^* - 1} P^{f(t^* - l)}(i,j) 
= \pi_i P(i,j)
$$

But as $\pi_j$ is the probability of seeing state $j$ after equilibrium, 
$\pi_j = \sum_i v_{ij} = \sum_i \pi_i p_{ij},$
and therefore $\pi$ is the stationary distribution for $P$.

(2) \textit{$P$ ergodic means $\GLAMP$ has equilibrium state:}
$\GLAMP$ can be expressed as a $k$th order Markov chain, with
transitions of the form
\[(x_{1}, \ldots, x_{k}) \rightarrow (x_{2}, x_{3}, \ldots,
  x_{k}, x'),
\]
with transition probability
\[ \sum_{i=1}^k w_i P^{f(k+1 - i)}(x_{k+1 -i}, x') 
= P(x_{k+1 -i}, x').
\]
Let $Q$ be the associated transition matrix on all $k$-tuples of
states reachable from start states of form $(x, \ldots, x)$. $Q$ is
thus connected by definition, and hence irreducible.

For aperiodicity, we need to show that the gcd of all cycles of $Q$ is
$1$. Suppose not, and that there is a $d > 1$ dividing the length of
all cycles in the underlying graph. $P$ is aperiodic, so there is some
cycle in $P$, say $x_1, \ldots, x_l, x_1$, with $l$ coprime to $d$.

If $k \leq l$, noting that $(x_{l -k + 1}, \ldots, x_l)$, which
is reachable
from $(x_{l -k}, \ldots, x_{l-k})$, is in our state space,
$$(x_{l -k + 1}, \ldots, x_l) \rightarrow (x_{l -k + 2}, \ldots, x_l, x_1) \rightarrow \cdots (x_{l -k + 1}, \ldots, x_l),$$
gives a cycle of length $l$ in $Q$.  If $k > l$, we adjust our start
state to
$$(x_1, \ldots, x_l,x_1, \ldots, x_l, \ldots, x_1, \ldots, x_r),$$
i.e., repeat $x_1, \ldots, x_l$ as many times as will fit, and add on
an initial segment equal to the remainder. (Note this is also
reachable, from say, $(x_l, \ldots, x_l)$.) Walking around as before
also gives us a cycle of length $l$. So $Q$ has equilibrium
$\tilde{\pi}$. We turn this into a distribution over single states $\pi$ by
summing elements of $\tilde{\pi}$ which have the same last state. This
precisely gives the probability of finding GLAMP at a particular
state.

(3) \textit{Equilibrium state same as that of $P$:} After showing that
$P$ ergodic means GLAMP has an equilibrium state $\pi$, we use (1) 
to finish the proof: by (1), $\pi$ is also an equilibrium state
for $P$.

\fi

\iffalse
\section{Examples}

To make the guarantees more concrete, we study some examples. 

%% \begin{tabular}{|l|c|c|} \hline
%% Monotonic threshold weights & $t/108$ & $t/5$ \\ \hline
%% Exponential decay & $t/6$ & $t/k$ \\ \hline
%% \end{tabular}

Our general strategy in providing bounds will be to lower bound 
$$  \displaystyle{\frac{\epsilon^2 E(W)}{(1 + \epsilon)(2 \sigma^2 + \frac{2}{3} k \epsilon E(W))}}$$

which appears in our expression for the probability from the previous section
$$  \exp\left(- \displaystyle{\frac{t \epsilon^2 E(W)}{(1 + \epsilon)(2 \sigma^2 + \frac{2}{3} k \epsilon E(W))}} \right) $$


\textbf{Monotonic Thresholded Weights}
Returning to our monotonic thresholded weights, we can explicitly calculate the mean and variance as
\begin{align*}
E(W) & \approx 2.5 \\
\sigma^2 & \approx 42 \\
\end{align*}

For large $k$, which is where our natural growth rate becomes especially important, we can afford to have $\epsilon = 1$ and not give too much away in terms of growth rate. Substituting in and calculating gives a value greater than $1/200$. So for $T \sim O(1000)$ (a small number for website visits, etc) for all $t \geq T$, with high probability, we have $e_t \geq t/2*E(W) \geq t/5$, much better than the naive $t/108$. \textbf{IS THE VALUE FOR $T$ REALLY A GOOD BOUND -- TOO LARGE??}

\textbf{Exponential Decay} Another popular choice for decreasing probabilities $w_1, w_2, \ldots,  w_k$ would be a truncated exponential decay:
$$ w_l = \frac{1}{C} e^{-\theta l} $$
where $C$ is a normalizing constant, and $\theta > 0$ controls the decay rate.

Noting that $E(W) \geq 1$, we have
$$ \displaystyle{\frac{\epsilon^2 E(W)}{(1 + \epsilon)(2 \sigma^2 + \frac{2}{3} k \epsilon E(W))}} \geq \displaystyle{\frac{\epsilon^2 }{(1 + \epsilon)(2 \sigma^2 + \frac{2}{3} k \epsilon E(W))}} $$

For large $k$, which is where our natural growth rate becomes especially important, we can afford to have $\epsilon = 1$ and not give too much away in terms of growth rate. Our expression to lower bound is thus
\[ \displaystyle{\frac{1 }{2(2 \sigma^2 + \frac{2}{3} k E(W))}}  \tag{*} \]

We can do this by providing upper bounds for $E(W)$ and $\sigma^2$. First note that
$$ E(W) = \frac{1}{C} \sum_{l = 1}^k l e^{-\theta l} $$But

$$ \sum_{l = 1}^k l e^{-\theta l} \leq \sum_{l = 1}^{\infty} e^{-\theta l} $$
But
$$ \sum_{l = 1}^{\infty} e^{-\theta l} = - \frac{d}{d \theta} \sum_{l=1}^{\infty} e^{-\theta l} $$
So summing the geometric series on the right hand side and differentiating, we have
$$ \sum_{l = 1}^{\infty} e^{-\theta l} = \frac{e^{\theta}}{(e^{\theta} - 1)^2} $$
Finally, by writing out $C$ explicitly, it easily follows that
$$ \frac{1}{C} \leq e^{\theta}$$
and so 
$$ E(W) \leq \left( \frac{e^{\theta}}{e^{\theta} - 1} \right)^2 $$

Looking at $\sigma^2$, we have
$$ \sigma^2 = \frac{1}{C} \sum_{l=1}^k l^2 e^{-\theta l} - E(W)^2 < \frac{1}{C} \sum_{l=1}^{\infty} l^2 e^{-\theta l} $$
But
$$ \sum_{l=1}^{\infty} l^2 e^{-\theta l} = \frac{d^2}{d \theta^2} \sum_{l=1}^{\infty} e^{-\theta l}  $$
and again writing the geometric series in closed form and differentiating twice gives
$$ \sum_{l=1}^{\infty} l^2 e^{-\theta l} = \frac{e^{\theta}(e^{\theta} + 1)}{(e^{\theta} - 1)^3} $$
And so
$$\sigma^2 < \frac{e^{2 \theta}(e^{\theta} + 1)}{(e^{\theta} - 1)^3} $$

For reasonable choices of $\theta$, e.g. $\theta = 1$, $E(W) < 3$ and $\sigma^2 < 5.5$, so (*) evaluates to $1/(22 + 4k)$, so for $T > 4k$, for all $ t \geq T$, with high probability, we see a growth rate of at least $t/2E(W) \geq t/6$, a marked improvement over the naive bound. 
\vspace{5mm}
\fi


